When LLM Rationales Become User-Facing: Effects on Trust Perception, Decision-Making, and Gaze Behaviors

Large language models (LLMs) increasingly show step-by-step reasoning rationales alongside their answers, turning reasoning from an internal model capability into a user-facing interface feature. Yet it is unclear whether such rationales help users judge when trust is warranted or merely persuade through fluent reasoning. We address this gap through the lens of auditable trust calibration: user-facing rationales should help people inspect whether an answer is warranted by evidence. We test this framing in factual verification through two linked studies. Study 1, an online experiment (N=68), manipulated rationale presentation format (instant, delayed, on demand), rationale correctness (correct, incorrect), and certainty framing (none, certain, uncertain). Study 2, a controlled eye-tracking study (N=54), examined how no-, correct-, and incorrect-rationale conditions were associated with users' trust, decision-making, and eye-movement patterns. Study 1 showed no reliable presentation-format effects; instead, rationale correctness and certainty framing influenced the trust in the information, trust in the LLM system, and decision confidence. In Study 2, incorrect rationales drew more attention to the supporting evidence and larger pupil diameter while the rationale was viewed, consistent with greater cognitive effort. Incorrect rationales also lowered trust in LLM system relative to showing no rationale, whereas the no-rationale difference was weaker for trust in information. A post-hoc predictive modeling analysis of gaze data from Study 2 further showed that gaze features carried predictive signal for trust- and decision-related user states. This work challenges the assumption that more reasoning is always better and supports rationale designs that are selective, linked to evidence, calibrated in how they express certainty, and easier to verify.

==> tables/lab_gaze_statistics.tex <==
% \begin{table}[!htbp]
% \centering
% \renewcommand{\arraystretch}{1.16}
% % \small % Reduce font size slightly for better fit
% \footnotesize
% \setlength{\tabcolsep}{0pt} % Slightly increase column separation for readability
% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}p{1.2cm}p{0.6cm}p{1.4cm}p{1.0cm}p{1.2cm}p{1.2cm}p{1.9cm}p{0.6cm}@{}}
% \hline

% \textbf{Gaze} & \textbf{AOI} & \textbf{Condition} & \textbf{Coeff} & \textbf{\revise{P (Orig)}} & \textbf{\revise{P (Corrected)}} & \textbf{Effect ($Std. \beta$)} & \textbf{Sig} \\ 
% \hline

% \multirow{9}{*}{\parbox{1.2cm}{Fixation Count}} 
%     & \multirow{3}{*}{AOI-1} 
%     & No Reasoning & -4.02 & \textbf{.033} & \textbf{.079} & .22 (medium) & - \\ \cline{3-8} 
%     & & Correct Reasoning & -4.54 & \textbf{.015} & \textbf{.055} & .25 (medium) & - \\ \cline{3-8} 
%     & & Incorrect Reasoning & 6.01 & .082 & .150 & .33 (medium) &  \\ \cline{2-8}
    
%     & \multirow{3}{*}{AOI-2} % GEE
%     & No Reasoning & 0.61 & .962 & .962 & .00 (small) &  \\ \cline{3-8} 
%     & & Correct Reasoning & -3.23 & .827 & .910 & .02 (small) &   \\ \cline{3-8} 
%     & & Incorrect Reasoning & 34.61 & \textbf{.036} & \textbf{.079} & .26 (medium) &  - \\ \cline{2-8}
    
%     & \multirow{3}{*}{AOI-3} 
%     & No Reasoning & -8.14 & .198 & .272 & .14 (small) &   \\ \cline{3-8} 
%     & & Correct Reasoning & 9.90 & .151 & .237 & .17 (small) &   \\ \cline{3-8} 
%     & & Incorrect Reasoning & -5.53 & .559 & .683 & .10 (small) &   \\ \hline


% \multirow{9}{*}{\parbox{1.8cm}{Fixation \\Duration}} 
%     & \multirow{3}{*}{AOI-1} 
%     & No Reasoning & -51.39 & \textbf{.000} & \textbf{.000} & .43 (large) &  ** \\ \cline{3-8} 
%     & & Correct Reasoning & -37.64 & \textbf{.006} & \textbf{.017} & .31 (medium) & * \\ \cline{3-8} 
%     & & Incorrect Reasoning & 71.27 & \textbf{.000} & \textbf{.000} & .59 (large) & ** \\ \cline{2-8}
    
%     & \multirow{3}{*}{AOI-2} 
%     & No Reasoning & 4.60 & \textbf{.038} & \textbf{.069} & .14 (medium) & - \\ \cline{3-8} 
%     & & Correct Reasoning & -2.80 & .218 & .343 & .09 (small) &   \\ \cline{3-8} 
%     & & Incorrect Reasoning & 1.75 & .584 & .642 & .05 (small) &   \\ \cline{2-8}
    
%     & \multirow{3}{*}{AOI-3} 
%     & No Reasoning & -0.46 & .879 & .879 & .01 (small) &   \\ \cline{3-8} 
%     & & Correct Reasoning & -1.61 & .553 & .642 & .05 (small) &   \\ \cline{3-8} 
%     & & Incorrect Reasoning & 2.85 & .519 & .642 & .09 (small) &   \\ \hline


% \multirow{9}{*}{\parbox{1.8cm}{Saccade Count}} 
%     & \multirow{3}{*}{AOI-1} 
%     & No Reasoning & -5.13 & \textbf{.044} & \textbf{.086} & .21 (medium) & - \\ \cline{3-8} 
%     & & Correct Reasoning & -7.38 & \textbf{.013} & \textbf{.047} & .26 (medium) & * \\ \cline{3-8} 
%     & & Incorrect Reasoning & 8.89 & \textbf{.047} & \textbf{.086} & .36 (medium) & - \\ \cline{2-8}
    
%     & \multirow{3}{*}{AOI-2} 
%     & No Reasoning & -4.35 & .787 & .787 & .03 (small) &   \\ \cline{3-8} 
%     & & Correct Reasoning & -7.82 & .651 & .716 & .05 (small) &   \\ \cline{3-8} 
%     & & Incorrect Reasoning & 43.77 & \textbf{.026} & \textbf{.071} & .28 (medium) & - \\ \cline{2-8}
    
%     & \multirow{3}{*}{AOI-3} 
%     & No Reasoning & -9.40 & .223 & .307 & .12 (medium) &   \\ \cline{3-8} 
%     & & Correct Reasoning & 10.71 & .160 & .251 & .14 (medium) &  \\ \cline{3-8} 
%     & & Incorrect Reasoning & -7.96 & .487 & .595 & .10 (medium) &   \\ \hline


% \multirow{9}{*}{\parbox{1.8cm}{Saccade Length}} 
%     & \multirow{3}{*}{AOI-1} 
%     & No Reasoning & 0.03 & .124 & .341 & .17 (medium) &   \\ \cline{3-8} 
%     & & Correct Reasoning & 0.01 &.531 & .649 & .08 (small) &   \\ \cline{3-8} 
%     & & Incorrect Reasoning & -0.07 & \textbf{.020} & \textbf{.073} & .38 (medium) & - \\ \cline{2-8}
    
%     & \multirow{3}{*}{AOI-2} 
%     & No Reasoning & 0.00 & .355 & .558 & .08 (small) &   \\ \cline{3-8} 
%     & & Correct Reasoning & 0.00 & .181 & .398 & .12 (medium) &   \\ \cline{3-8} 
%     & & Incorrect Reasoning & 0.00 & .829 & .829 & .02 (small) &   \\ \cline{2-8}
    
%     & \multirow{3}{*}{AOI-3} 
%     & No Reasoning & 0.00 & .276 & .506 & .08 (small) &   \\ \cline{3-8} 
%     & & Correct Reasoning & 0.00 & .456 & .627 & .06 (small) &   \\ \cline{3-8} 
%     & & Incorrect Reasoning & 0.00 & .685 & .754 & .05 (small) &   \\ \hline


% \multirow{9}{*}{\parbox{1.8cm}{Pupil\\Diameter\\Fixation}} 
%     & \multirow{3}{*}{AOI-1} 
%     & No Reasoning & -0.41 & \textbf{.002} & \textbf{.011} & .35 (medium) & * \\ \cline{3-8} 
%     & & Correct Reasoning & -0.33 & \textbf{.018} & \textbf{.040} & .29 (medium) & * \\ \cline{3-8} 
%     & & Incorrect Reasoning & 0.50 & \textbf{.003} & \textbf{.011} & .43 (large) &  * \\ \cline{2-8}
    
%     & \multirow{3}{*}{AOI-2} 
%     & No Reasoning & 0.00 & .673 & .823 & .01 (small) &   \\ \cline{3-8} 
%     & & Correct Reasoning & 0.01 & .445 & .699 & .02 (small) &   \\ \cline{3-8} 
%     & & Incorrect Reasoning & 0.00 & .898 & .932 & .00 (small) &   \\ \cline{2-8}
    
%     & \multirow{3}{*}{AOI-3} 
%     & No Reasoning & 0.00 & .227 & .416 & .03 (small) &   \\ \cline{3-8} 
%     & & Correct Reasoning & 0.01 & .531 & .730 & .01 (small) &   \\ \cline{3-8} 
%     & & Incorrect Reasoning & 0.00 & .932 & .932 & .00 (small) &   \\ 
% \bottomrule    
% \end{tabular*}
% % \Description{Table 7: Result of GEE analysis on eye tracking data from the lab study. No Reasoning: Human vs. LLM) Correct Reasoning: Human vs. AI)}
% \caption{Results from the GEE analysis \revise{with False Discovery Rate (FDR) correction} on the eye tracking data. (**$p$<.01, *$p$<.05, -$p$<.10)}
% \Correct Reasoning{tab:gaze-results}
% \vspace{-3.2mm}
% \end{table}



\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.1}
\footnotesize
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}p{0.4cm}p{0.8cm}p{2.0cm}p{1.0cm}p{1.4cm}p{1.6cm}p{1.8cm}p{0.6cm}@{}}
\toprule
\textbf{Gaze} & \textbf{AOI} & \textbf{Condition} & \textbf{Coeff} & \textbf{P (Original)} & \textbf{P (Corrected)} & \textbf{Effect ($\boldsymbol{\beta}$)} & \textbf{Sig} \\
\midrule

% Fixation Count
\multirow{9}{*}{\rotatebox{90}{\textbf{Fixation Count}}} 
    & \multirow{3}{*}{AOI-1} 
        & No Reasoning & $-4.02$ & \textbf{.033} & \textbf{.079} & .22 (medium) & - \\
        & & Correct Reasoning & $-4.54$ & \textbf{.015} & \textbf{.055} & .25 (medium) & - \\
        & & Incorrect Reasoning & $6.01$ & .082 & .150 & .33 (medium) & \\
    \cmidrule(lr){2-8}
    
    & \multirow{3}{*}{AOI-2} 
        & No Reasoning & $0.61$ & .962 & .962 & .00 (small) & \\
        & & Correct Reasoning & $-3.23$ & .827 & .910 & .02 (small) & \\
        & & Incorrect Reasoning & $34.61$ & \textbf{.036} & \textbf{.079} & .26 (medium) & - \\
    \cmidrule(lr){2-8}
    
    & \multirow{3}{*}{AOI-3} 
        & No Reasoning & $-8.14$ & .198 & .272 & .14 (small) & \\
        & & Correct Reasoning & $9.90$ & .151 & .237 & .17 (small) & \\
        & & Incorrect Reasoning & $-5.53$ & .559 & .683 & .10 (small) & \\
\midrule

% Fixation Duration
\multirow{9}{*}{\rotatebox{90}{\textbf{Fixation Duration}}} 
    & \multirow{3}{*}{AOI-1} 
        & No Reasoning & $-51.39$ & \textbf{.000} & \textbf{.000} & .43 (large) & ** \\
        & & Correct Reasoning & $-37.64$ & \textbf{.006} & \textbf{.017} & .31 (medium) & * \\
        & & Incorrect Reasoning & $71.27$ & \textbf{.000} & \textbf{.000} & .59 (large) & ** \\
    \cmidrule(lr){2-8}
    
    & \multirow{3}{*}{AOI-2} 
        & No Reasoning & $4.60$ & \textbf{.038} & \textbf{.069} & .14 (medium) & - \\
        & & Correct Reasoning & $-2.80$ & .218 & .343 & .09 (small) & \\
        & & Incorrect Reasoning & $1.75$ & .584 & .642 & .05 (small) & \\
    \cmidrule(lr){2-8}
    
    & \multirow{3}{*}{AOI-3} 
        & No Reasoning & $-0.46$ & .879 & .879 & .01 (small) & \\
        & & Correct Reasoning & $-1.61$ & .553 & .642 & .05 (small) & \\
        & & Incorrect Reasoning & $2.85$ & .519 & .642 & .09 (small) & \\
\midrule

% Saccade Count
\multirow{9}{*}{\rotatebox{90}{\textbf{Saccade Count}}} 
    & \multirow{3}{*}{AOI-1} 
        & No Reasoning & $-5.13$ & \textbf{.044} & \textbf{.086} & .21 (medium) & - \\
        & & Correct Reasoning & $-7.38$ & \textbf{.013} & \textbf{.047} & .26 (medium) & * \\
        & & Incorrect Reasoning & $8.89$ & \textbf{.047} & \textbf{.086} & .36 (medium) & - \\
    \cmidrule(lr){2-8}
    
    & \multirow{3}{*}{AOI-2} 
        & No Reasoning & $-4.35$ & .787 & .787 & .03 (small) & \\
        & & Correct Reasoning & $-7.82$ & .651 & .716 & .05 (small) & \\
        & & Incorrect Reasoning & $43.77$ & \textbf{.026} & \textbf{.071} & .28 (medium) & - \\
    \cmidrule(lr){2-8}
    
    & \multirow{3}{*}{AOI-3} 
        & No Reasoning & $-9.40$ & .223 & .307 & .12 (medium) & \\
        & & Correct Reasoning & $10.71$ & .160 & .251 & .14 (medium) & \\
        & & Incorrect Reasoning & $-7.96$ & .487 & .595 & .10 (medium) & \\
\midrule

% Saccade Length
\multirow{9}{*}{\rotatebox{90}{\textbf{Saccade Length}}} 
    & \multirow{3}{*}{AOI-1} 
        & No Reasoning & $0.03$ & .124 & .341 & .17 (medium) & \\
        & & Correct Reasoning & $0.01$ & .531 & .649 & .08 (small) & \\
        & & Incorrect Reasoning & $-0.07$ & \textbf{.020} & \textbf{.073} & .38 (medium) & - \\
    \cmidrule(lr){2-8}
    
    & \multirow{3}{*}{AOI-2} 
        & No Reasoning & $0.00$ & .355 & .558 & .08 (small) & \\
        & & Correct Reasoning & $0.00$ & .181 & .398 & .12 (medium) & \\
        & & Incorrect Reasoning & $0.00$ & .829 & .829 & .02 (small) & \\
    \cmidrule(lr){2-8}
    
    & \multirow{3}{*}{AOI-3} 
        & No Reasoning & $0.00$ & .276 & .506 & .08 (small) & \\
        & & Correct Reasoning & $0.00$ & .456 & .627 & .06 (small) & \\
        & & Incorrect Reasoning & $0.00$ & .685 & .754 & .05 (small) & \\
\midrule

% Pupil Diameter Fixation
\multirow{9}{*}{\rotatebox{90}{\textbf{Pupil Diameter}}} 
    & \multirow{3}{*}{AOI-1} 
        & No Reasoning & $-0.41$ & \textbf{.002} & \textbf{.011} & .35 (medium) & * \\
        & & Correct Reasoning & $-0.33$ & \textbf{.018} & \textbf{.040} & .29 (medium) & * \\
        & & Incorrect Reasoning & $0.50$ & \textbf{.003} & \textbf{.011} & .43 (large) & * \\
    \cmidrule(lr){2-8}
    
    & \multirow{3}{*}{AOI-2} 
        & No Reasoning & $0.00$ & .673 & .823 & .01 (small) & \\
        & & Correct Reasoning & $0.01$ & .445 & .699 & .02 (small) & \\
        & & Incorrect Reasoning & $0.00$ & .898 & .932 & .00 (small) & \\
    \cmidrule(lr){2-8}
    
    & \multirow{3}{*}{AOI-3} 
        & No Reasoning & $0.00$ & .227 & .416 & .03 (small) & \\
        & & Correct Reasoning & $0.01$ & .531 & .730 & .01 (small) & \\
        & & Incorrect Reasoning & $0.00$ & .932 & .932 & .00 (small) & \\
\bottomrule
\end{tabular*}
\vspace{0.6mm}
\caption{Results from the GEE analysis with False Discovery Rate (FDR) correction on the eye tracking data. (**$p$<.01, *$p$<.05, -$p$<.10)}
\label{tab:gaze-results}
% \vspace{-2mm}
\end{table}

==> tables/online_demographics.tex <==
\begin{table}[!h]
\centering
\footnotesize
\renewcommand{\arraystretch}{0.49}
\begin{tabularx}{\columnwidth}{p{1cm} >{\raggedright\arraybackslash}p{1cm} >{\raggedright\arraybackslash}X}
\toprule
\textbf{Demographic} & \textbf{Categories} & \textbf{Numbers of Participants (\%)} \\
\midrule
Gender & & 
\\ 
 & Female & 0 (.0\%)
\\ 
 & Male & 0 (.0\%)
\\
 % & Non-binary & 0 (.0\%)
\hline
Age & & 
\\
 & 18-24 & 0 (.0\%)
\\
 & 25-34 & 0 (.0\%)
\\
 & 35-44 & 0 (.0\%)
\\
 & 45-54 & 0 (.0\%)
\\
 & 65+ & 0 (.0\%)
\\

\hline
Education & & 
\\
 & High school degree or equivalent & 0 (.0\%)
\\
 & Bachelor’s degree & 0 (.0\%)
\\
 & Master’s degree & 0 (.0\%)
\\
 & Doctorate or higher & 0 (.0\%)
\\
\bottomrule
\end{tabularx}
\vspace{0.36mm}
\caption{Characteristics of participants in the Study 1.}
\vspace{-5mm}
\label{table:online_demographics}
\end{table}


==> tables/survey_anova.tex <==

% \begin{table}[!htbp]
% \centering
% \footnotesize
% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llccc@{}}
% \toprule
% \textbf{Category} & \textbf{Variable} & \textbf{Effect Size} & \textbf{P-Value} & \textbf{Significance} \\ 
% \midrule
% \multirow{3}{*}{\textbf{Trust Info}}   
%                   & Strategy    & .618 & .539 & ns \\
%                   & Confidence Cue  & 4.778 & .009 & $**$ \\
%                   & Correctness & 4.552 & .034 & $*$ \\ 
% \hline

% \multirow{3}{*}{\textbf{Trust Meter}}    
%                   & Strategy    & 1.150 & .318 & ns \\
%                   & Confidence Cue  & 5.471 & .005 & $**$ \\
%                   & Correctness & 8.446 & .004 & $**$ \\ 

% \hline

% \multirow{3}{*}{\textbf{Trust System}} 
%                   & Strategy    & .313 & .731 & ns \\
%                   & Confidence Cue  & 3.097 & .021 & $*$ \\
%                   & Correctness & 4.552 & .125 & ns \\ 
% \hline

% \multirow{3}{*}{\textbf{Cognitive Load}}    
%                   & Strategy    & .786 & .456 & ns \\
%                   & Confidence Cue  & .167 & .846 & ns \\
%                   & Correctness & 2.194 & .139 & ns \\ 
% \hline

% \multirow{3}{*}{\textbf{Decision Confidence}}    
%                   & Strategy    & .327 & .721 & ns \\
%                   & Confidence Cue  & 6.524 & .002 & $**$ \\
%                   & Correctness & .283 & .595 & ns \\ 

% % \multirow{3}{*}{\textbf{Decision Performance}}    
% %                   & Strategy    & / & / & / \\ 
% %                   & Confidence Cue  & / & / & --- \\
% %                   & Correctness & --- & --- & --- \\ 

% \bottomrule
% \end{tabular*}

% \caption{Result of mix-ANOVA analysis.}
% \label{tab:survey_anova}
% \end{table}


\begin{table*}[!htbp]
\centering
\scriptsize
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{3pt}
\caption{\emph{Study 1 trial-level factorial model results.} Entries report cluster-robust Wald statistics with raw $p$ values for the presentation, certainty, correctness, and interaction terms. Continuous outcomes were fit with linear models and advice adoption with a binomial generalized linear model; all models included stimulus fixed effects and participant-clustered standard errors. The term-test degrees of freedom were 2, 2, 1, 4, 2, 2, and 4, respectively.}
\vspace{-1.6mm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Outcome} & \textbf{Presentation} & \textbf{Certainty} & \textbf{Correctness} & \textbf{Format$\times$Certainty} & \textbf{Format$\times$Correctness} & \textbf{Certainty$\times$Correctness} & \textbf{Three-way} \\
\midrule
Trust in information & 0.80 (.672) & 5.60 (.061) & 5.56 (.018) & 2.78 (.596) & 0.85 (.653) & 2.43 (.296) & 5.36 (.252) \\
Trust in LLM system & 0.70 (.703) & 7.91 (.019) & 4.75 (.029) & 1.47 (.833) & 0.44 (.804) & 1.45 (.485) & 1.97 (.742) \\
Decision confidence & 0.27 (.876) & 3.44 (.179) & 3.86 (.049) & 5.63 (.229) & 0.63 (.729) & 1.56 (.458) & 8.34 (.080) \\
Advice adoption & 3.00 (.223) & 1.09 (.580) & 1.56 (.212) & 3.81 (.432) & 0.87 (.647) & 1.69 (.430) & 1.80 (.773) \\
Manipulation check & 0.52 (.769) & 7.73 (.021) & 6.79 (.009) & 2.06 (.724) & 1.39 (.500) & 2.55 (.279) & 7.35 (.119) \\
\bottomrule
\end{tabular}}
\label{tab:survey_anova}
\end{table*}

==> tables/umap_pred.tex <==
% % preamble 里确保有：
% % \usepackage{booktabs,multirow,tabularx,array}

% \begin{table*}[!ht]
% \centering
% \scriptsize
% \renewcommand{\arraystretch}{1.16}
% \setlength{\tabcolsep}{1pt}

% % 左对齐 + 自动换行列类型
% \newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
% % 均分列（左对齐 + 自动换行）
% \newcolumntype{Y}{>{\raggedright\arraybackslash}X}

% \begin{tabularx}{\textwidth}{@{} L{1.2cm} L{0.72cm} *{15}{Y} @{}}
% \toprule
% \multirow{2}{*}{\textbf{Features}}
% & \multirow{2}{*}{\textbf{Models}}
% & \multicolumn{5}{c}{\textbf{Cognitive Load}}
% & \multicolumn{5}{c}{\textbf{Decision Confidence}}
% & \multicolumn{5}{c}{\textbf{Decision Accuracy}} \\
% \cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17}
% & &
% \textbf{All} & \textbf{No} & \textbf{Corr} & \textbf{Incorr} & \textbf{MoE}
% & \textbf{All} & \textbf{No} & \textbf{Corr} & \textbf{Incorr} & \textbf{MoE}
% & \textbf{All} & \textbf{No} & \textbf{Corr} & \textbf{Incorr} & \textbf{MoE} \\
% \midrule


% \multirow{8}{*}{\makecell[l]{Eye-tracking\\Only}}
% & LR & .61/.65/.64 & .61/.57/.68 & .50/.51/.52 & \underline{.63/.60/.62} & .58/.63/.63 & .62/.69/.63 & .63/.66/.68 & .60/.68/.58 & .59/.68/.59 & .58/.66/.57 & .57/.69/.59 & .56/.67/.53 & .52/.65/.51 & .54/.68/.48 & \underline{.61/.73/.54} \\
% & SVM      & .62/.76/.51 & .57/.64/.52 & .60/.75/.55 & .49/.45/.48 & \underline{.62/.76/.52} & .65/.78/.59 & .66/.70/.56 & .67/.79/.59 & .68/.81/.54 & .65/.77/.52 & .79/.88/.49 & .78/.87/.41 & .78/.87/.44 & \underline{.83/.91/.46} & .79/.88/.47 \\
% & RF & \underline{.66/.74/.68} & .64/.64/.68 & .58/.67/.58 & .60/.60/.61 & .64/.74/.62 & .65/.76/.67 & .67/.67/.70 & .71/.81/.67 & .67/.78/.65 & .67/.77/.66 & .79/.88/.62 & .76/.86/.47 & .74/.85/.55 & \underline{.82/.90/.57} & .79/.88/.58 \\
% & ET      & \underline{.65/.74/.68} & .63/.62/.68 & .58/.68/.57 & .55/.51/.61 & .62/.72/.63 & .65/.77/.66 & .63/.70/.69 & \underline{.71/.81/.66} & .66/.77/.65 & .66/.77/.65 & .79/.88/.62 & .76/.86/.61 & .75/.86/.50 & \underline{.82/.90/.61} & .79/.88/.60 \\
% & AdaB      & \underline{.62/.73/.63} & .63/.62/.67 & .60/.75/.52 & .57/.51/.57 & .61/.70/.60 & .67/.79/.64 & .59/.66/.61 & \underline{.70/.82/.65} & .67/.80/.52 & .61/.72/.59 & .79/.88/.57 & .74/.85/.54 & .76/.87/.50 & .83/.90/.53 & .75/.85/.55 \\
% & XGB         & .64/.75/.63 & \underline{.67/.75/.68} & .66/.67/.69 & .58/.87/.74 & .61/.85/.70 & .60/.70/.60 & \underline{.74/.85/.62} & .62/.85/.57 & .67/.75/.68 & .71/.84/.47 & .71/.84/.60 & \underline{.82/.90/.59} & .67/.79/.62 & .62/.90/.59 & .63/.70/.60 \\
% & MLP      & \underline{.64/.74/.62} & .58/.60/.62 & .54/.65/.52 & .57/.60/.60 & .57/.66/.59 & .65/.76/.64 & .64/.70/.65 & \underline{.65/.77/.54} & .63/.74/.57 & .59/.69/.58 & \underline{.79/.88/.54} & .72/.83/.51 & .67/.79/.43 & .79/.88/.48 & .70/.82/.53 \\
% & GPC   & .64/.76/.64 & \underline{.67/.83/.73} & .60/.68/.61 & .54/.75/.54 & .60/.87/.73 & .61/.83/.73 & .61/.71/.61 & .60/.68/.56 & .67/.79/.64 & \underline{.72/.73/.68} & .64/.83/.73 & .67/.83/.73 & .57/.75/.54 & \underline{.83/.91/.58} & .61/.83/.73 \\
% \midrule


% \multirow{8}{*}{\makecell[l]{User Priors\\Only}}
% & LR   & \multicolumn{5}{c}{.65/.69/.68} & \multicolumn{5}{c}{.57/.64/.61} & \multicolumn{5}{c}{.60/.71/.62} \\
% & SVM  & .73/.80/.68 & .73/.80/.68 & .73/.80/.68 & .73/.80/.68 & .73/.80/.68 & .65/.78/.57 & .65/.78/.57 & .65/.78/.57 & .65/.78/.57 & .65/.78/.57 & .80/.88/.61 & .80/.88/.61 & .80/.88/.61 & .80/.88/.61 & .80/.88/.61 \\
% & RF & .70/.76/.73 & .70/.76/.73 & .70/.76/.73 & .70/.76/.73 & .70/.76/.73 & .59/.66/.63 & .59/.66/.63 & .59/.66/.63 & .59/.66/.63 & .59/.66/.63 & .67/.77/.64 & .67/.77/.64 & .67/.77/.64 & .67/.77/.64 & .67/.77/.64 \\
% & ET      & .73/.79/.73 & .73/.79/.73 & .73/.79/.73 & .73/.79/.73 & .73/.79/.73 & .65/.75/.63 & .65/.75/.63 & .65/.75/.63 & .65/.75/.63 & .65/.75/.63 & .80/.88/.62 & .80/.88/.62 & .80/.88/.62 & .80/.88/.62 & .80/.88/.62 \\
% & AdaB      & .71/.78/.72 & .71/.78/.72 & .71/.78/.72 & .71/.78/.72 & .71/.78/.72 & .64/.78/.59 & .64/.78/.59 & .64/.78/.59 & .64/.78/.59 & .64/.78/.59 & .79/.88/.60 & .79/.88/.60 & .79/.88/.60 & .79/.88/.60 & .79/.88/.60 \\
% & XGB         & .63/.78/.62 & .63/.78/.62 & .63/.78/.62 & .63/.78/.62 & .63/.78/.62 & .80/.88/.63 & .80/.88/.63 & .80/.88/.63 & .80/.88/.63 & .80/.88/.63 & .73/.79/.73 & .73/.79/.73 & .73/.79/.73 & .73/.79/.73 & .73/.79/.73 \\
% & MLP      & .64/.74/.67 & .64/.74/.67 & .64/.74/.67 & .64/.74/.67 & .64/.74/.67 & .62/.75/.54 & .62/.75/.54 & .62/.75/.54 & .62/.75/.54 & .62/.75/.54 & .79/.88/.58 & .79/.88/.58 & .79/.88/.58 & .79/.88/.58 & .79/.88/.58 \\
% & GPC            & .65/.78/.55 & .65/.78/.55 & .65/.78/.55 & .65/.78/.55 & .65/.78/.55 & .79/.88/.61 & .79/.88/.61 & .79/.88/.61 & .79/.88/.61 & .79/.88/.61 & .73/.80/.74 & .73/.80/.74 & .73/.80/.74 & .73/.80/.74 & .73/.80/.74 \\
% \midrule


% \multirow{8}{*}{\makecell[l]{Multimodal\\Fusion}}
% & LR & .66/.71/.73 & .65/.64/.70 & .58/.63/.62 & \underline{.70/.72/.74} & .65/.71/.69 & .62/.68/.66 & \underline{.69/.72/.73} & .58/.68/.54 & .62/.71/.60 & .60/.68/.60 & .64/.75/.62 & .59/.71/.54 & .66/.77/.57 & \underline{.68/.79/.55}& .67/.78/.60 \\
% & SVM      & \underline{.66/.76/.51} & .57/.63/.52 & .60/.75/.56 & .49/.45/.48 & .61/.76/.52 & .63/.76/.60 & .66/.70/.56 & \underline{.68/.80/.60} & .68/.81/.54 & .65/.77/.52 & .79/.88/.49 & .78/.87/.41 & .77/.87/.41 & \underline{.83/.91/.49} & .79/.88/.47 \\
% & RF & \underline{.71/.78/.76} & .67/.67/.72 & .59/.69/.62 & .63/.62/.66 & .65/.75/.67 & .66/.77/.68 & .67/.71/.73 & \underline{.71/.81/.69} & .67/.78/.65 & .67/.77/.67 & .79/.88/.64 & .76/.86/.51 & .76/.86/.56 & \underline{.84/.91/.57} & .79/.88/.61 \\
% & ET      & .65/.81/.79 & .\underline{69/.69/.74} & .63/.72/.67 & .68/.75/.72 & .68/.75/.72 & .67/.77/.66 & .68/.71/.74 & \underline{.74/.83/.70} & .68/.77/.61 & .67/.77/.68 & .79/.77/.66 & .78/.87/.61 & .74/.84/.60 & \underline{.81/.89/.57} & .77/.87/.61 \\
% & AdaB      & .65/.74/.67 & \underline{.67/.68/.68} & .60/.72/.52 & .57/.52/.56 & .63/.71/.63 & .68/.78/.65 & .62/.68/.65 & \underline{.70/.81/.64} & .66/.79/.53 & .63/.74/.61 & .79/.88/.56 & .76/.86/.51 & .76/.87/.52 & .83/.90/.53 & .73/.84/.55 \\
% & XGB         & .65/.77/.58 & .65/.77/.58 & .65/.77/.58 & .65/.77/.58 & .66/.85/.71 & .71/.86/.57 & .67/.72/.70 & .60/.71/.66 & \underline{.75/.86/.47} & .74/.83/.72 & .56/.71/.60 & \underline{.83/.91/.57} & .65/.77/.60 & .56/.71/.62 & .62/.73/.62 \\
% & MLP      & \underline{.73/.79/.76} & .61/.59/.67 & .46/.51/.47 & .62/.61/.65 & .62/.73/.62 & .65/.75/.63 & .66/.70/.71 & \underline{.74/.83/.62} & .66/.78/.58 & .66/.76/.64 & .79/.88/.55 & .73/.84/.53 & .71/.82/.54 & \underline{.85/.91/.51} & .78/.87/.62 \\
% & GPC   & .67/.80/.74 & .67/.80/.74 & .67/.80/.74 & .67/.80/.74 & .66/.83/.73 & .64/.73/.66 & .63/.73/.63 & .67/.73/.65 & \underline{.70/.74/.55} & .67/.73/.65 & .69/.80/.74 & .67/.80/.74 & .59/.73/.50 & \underline{.83/.91/.59} & .64/.73/.66 \\
% \bottomrule
% \end{tabularx}
% \caption{
% \textbf{Prediction results under different feature sets and AI conditions.} 
% Binary classification performance \textcolor{red}{(Accuracy/F1/AUC)} for predicting \textit{cognitive load}, \textit{decision confidence}, and \textit{decision accuracy}. 
% We compare three feature settings: \textit{Eye-tracking only}, \textit{User priors only}, and \textit{Multimodal fusion} (eye tracking + user priors), across multiple classifiers. 
% For each predicted target, we report overall performance on pooled trials (\textit{All}) and condition-stratified performance on \textit{No-AI}, \textit{Correct-AI}, and \textit{Incorrect-AI} trials; \textit{MoE} denotes a condition-aware mixture-of-experts baseline. 
% Best scores within each column are highlighted.}
% % \underline{Bold}: highest per column; \best{Red}: best overall per outcome.
% \label{tab:res_predictions}
% \vspace{-2.6mm}
% \end{table*}


% & \multicolumn{3}{c|}{\cellcolor{gray!20}\textbf{Rationale Format}} 
% & \multicolumn{3}{c|}{\cellcolor{blue!10}\textbf{Certainty Cue}} 
% & \multicolumn{2}{c}{\cellcolor{red!10}\textbf{Rationale Correctness}} \\


\begin{table*}[!ht]
\centering
\footnotesize
\renewcommand{\arraystretch}{0.74}
\setlength{\tabcolsep}{2pt}

% 左对齐 + 自动换行列类型
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
% 均分列（左对齐 + 自动换行）
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}

% 现在数据列变为：Eye(5) + Priors(1) + Fusion(5) = 11 列
\begin{tabularx}{\textwidth}{@{} L{1.4cm} L{0.86cm} *{11}{Y} @{}}
\toprule
\multirow{2}{*}{\textbf{Targets}}
& \multirow{2}{*}{\textbf{Models}}
& \multicolumn{5}{c}{\colorbox{gray!18}{\textbf{Eye-tracking Only}}}
& \multicolumn{1}{c}{\colorbox{blue!10}{\textbf{User Priors}}}
& \multicolumn{5}{c}{\colorbox{red!10}{\textbf{Multimodal Fusion}}}\\
\cmidrule(lr){3-7} \cmidrule(lr){8-8} \cmidrule(lr){9-13}
& &
\textbf{All} & \textbf{No} & \textbf{Corr} & \textbf{Incorr} & \textbf{MoE}
& \textbf{All}
& \textbf{All} & \textbf{No} & \textbf{Corr} & \textbf{Incorr} & \textbf{MoE} \\
\midrule

% ===================== Cognitive Load =====================
\multirow{7}{*}{\textbf{\makecell[l]{Cognitive\\Load}}}
& LR  & .61/.65/.64 & .61/.57/.68 & .50/.51/.52 & \underline{.63/.60/.62} & .58/.63/.63
      & .65/.69/.68
      & .66/.71/.73 & .65/.64/.70 & .58/.63/.62 & \underline{.70/.72/.74} & .65/.71/.69 \\
& SVM & .62/.76/.51 & .57/.64/.52 & .60/.75/.55 & .49/.45/.48 & \underline{.62/.76/.52}
      & .68/.75/.63
      & \underline{.66/.76/.51} & .57/.63/.52 & .60/.75/.56 & .49/.45/.48 & .61/.76/.52 \\
& RF  & \underline{.66/.74/.68} & .64/.64/.68 & .58/.67/.58 & .60/.60/.61 & .64/.74/.62
      & .65/.71/.68
      & \underline{.71/.78/.76} & .67/.67/.72 & .59/.69/.62 & .63/.62/.66 & .65/.75/.67 \\
& ET  & \underline{.65/.74/.68} & .63/.62/.68 & .58/.68/.57 & .55/.51/.61 & .62/.72/.63
      & .68/.74/.68
      & .65/.81/.79 & .\underline{69/.69/.74} & .63/.72/.67 & .68/.75/.72 & .68/.75/.72 \\
& AdaB& \underline{.62/.73/.63} & .63/.62/.67 & .60/.75/.52 & .57/.51/.57 & .61/.70/.60
      & .66/.73/.67
      & .65/.74/.67 & \underline{.67/.68/.68} & .60/.72/.52 & .57/.52/.56 & .63/.71/.63 \\
& XGB & \best{.66/.75/.69} &.61/.64/.66 & .57/.69/.60 & .62/.59/.63 & .60/.70/.60 
      & \best{.68/.73/.67}
      & \underline{.69/.77/.74} & .65/.66/.70 & .60/.71/.60 & .56/.56/.62 & .63/.71/.62 \\
& MLP & \underline{.64/.74/.62} & .58/.60/.62 & .54/.65/.52 & .57/.60/.60 & .57/.66/.59
      & .64/.74/.67
      & \best{.73/.79/.76} & .61/.59/.67 & .46/.51/.47 & .62/.61/.65 & .62/.73/.62 \\
% & GPC & .64/.76/.64 & \best{.67/.83/.73} & .60/.68/.61 & .54/.75/.54 & .60/.87/.73
%       & .73/.80/.73
%       & \underline{.67/.80/.74} & .67/.80/.74 & .67/.80/.74 & .67/.80/.74 & .66/.83/.73 \\
\midrule

% ===================== Decision Confidence =====================
\multirow{7}{*}{\textbf{\makecell[l]{Decision\\Confidence}}}
& LR  & .62/.69/.63 & \underline{.63/.66/.68} & .60/.68/.58 & .59/.68/.59 & .58/.66/.57
      & .57/.64/.61
      & .62/.68/.66 & \underline{.69/.72/.73} & .58/.68/.54 & .62/.71/.60 & .60/.68/.60 \\
& SVM & .65/.78/.59 & .66/.70/.56 & .67/.79/.59 & \underline{.68/.81/.54} & .65/.77/.52
      & .65/.78/.57
      & .63/.76/.60 & .66/.70/.56 & \underline{.68/.80/.60} & .68/.81/.54 & .65/.77/.52 \\
& RF  & .65/.76/.67 & .67/.67/.70 & \underline{.71/.81/.67} & .67/.78/.65 & .67/.77/.66
      & .59/.66/.63
      & .66/.77/.68 & .67/.71/.73 & \underline{.71/.81/.69} & .67/.78/.65 & .67/.77/.67 \\
& ET  & .65/.77/.66 & .63/.70/.69 & \underline{.71/.81/.66} & .66/.77/.65 & .66/.77/.65
      & .65/.75/.63
      & .67/.77/.66 & .68/.71/.74 & \underline{.74/.83/.70} & .68/.77/.61 & .67/.77/.68 \\
& AdaB& .67/.79/.64 & .59/.66/.61 & \underline{.70/.82/.65} & .67/.80/.52 & .61/.72/.59
      & .64/.78/.59
      & .68/.78/.65 & .62/.68/.65 & \underline{.70/.81/.64} & .66/.79/.53 & .63/.74/.61 \\
& XGB & .63/.75/.65 & .61/.67/.69 & \best{.71/.81/.69} & .67/.79/.62 & .65/.75/.64
      & \best{.65/.78/.62}
      & .64/.75/.68 & .68/.72/.71 & \best{.74/.83/.72} & .65/.77/.60 & .63/.73/.62 \\
& MLP & .65/.76/.64 & .64/.70/.65 & \underline{.65/.77/.54} & .63/.74/.57 & .59/.69/.58
      & .62/.75/.54
      & .65/.75/.63 & .66/.70/.71 & \underline{.74/.83/.62} & .66/.78/.58 & .66/.76/.64 \\
% & GPC & .61/.83/.73 & .61/.71/.61 & .60/.68/.56 & .67/.79/.64 & \underline{.72/.73/.68}
%       & .65/.78/.55
%       & .64/.73/.66 & .63/.73/.63 & .67/.73/.65 & \underline{.70/.74/.55} & .67/.73/.65 \\
\midrule

% ===================== Decision Accuracy =====================
\multirow{7}{*}{\textbf{\makecell[l]{Decision\\Accuracy}}}
& LR  & .57/.69/.59 & .56/.67/.53 & .52/.65/.51 & .54/.68/.48 & \underline{.61/.73/.54}
      & .60/.71/.62
      & .64/.75/.62 & .59/.71/.54 & .66/.77/.57 & \underline{.68/.79/.55}& .67/.78/.60 \\
& SVM & .79/.88/.49 & .78/.87/.41 & .78/.87/.44 & \underline{.83/.91/.46} & .79/.88/.47
      & .80/.88/.61
      & .79/.88/.49 & .78/.87/.41 & .77/.87/.41 & \underline{.83/.91/.49} & .79/.88/.47 \\
& RF  & .79/.88/.62 & .76/.86/.47 & .74/.85/.55 & \underline{.82/.90/.57} & .79/.88/.58
      & .67/.77/.64
      & .79/.88/.64 & .76/.86/.51 & .76/.86/.56 & \underline{.84/.91/.57} & .79/.88/.61 \\
& ET  & .79/.88/.62 & .76/.86/.61 & .75/.86/.50 & \best{.82/.90/.61} & .79/.88/.60
      & .80/.88/.62
      & .79/.77/.66 & .78/.87/.61 & .74/.84/.60 & \underline{.81/.89/.57} & .77/.87/.61 \\
& AdaB& .79/.88/.57 & .74/.85/.54 & .76/.87/.50 & \underline{.82/.90/.53} & .75/.85/.55 & .79/.88/.60 & .79/.88/.56 & .76/.86/.51 & .76/.87/.52 & \underline{.83/.90/.53} & .73/.84/.55 \\
& XGB & .78/.88/.62 & .77/.87/.58 & .73/.84/.47 & .82/.90/.59 & .74/.85/.57
      & \best{.80/.88/.63}
      & .78/.88/.65 & .76/.86/.57 & .75/.86/.47 & .83/.91/.57 & .75/.85/.56 \\
& MLP & \underline{.79/.88/.54} & .72/.83/.51 & .67/.79/.43 & .79/.88/.48 & .70/.82/.53
      & .79/.88/.58
      & .79/.88/.55 & .73/.84/.53 & .71/.82/.54 & \best{.85/.91/.58} & .78/.87/.62 \\
% & GPC & .64/.83/.73 & .67/.83/.73 & .57/.75/.54 & \best{.82/.90/.52} & .61/.83/.73
%       & .79/.88/.61
%       & .69/.80/.74 & .67/.80/.74 & .59/.73/.50 & \underline{.83/.91/.59} & .64/.73/.66 \\
\bottomrule
\end{tabularx}

\vspace{-0.0mm}
\caption{
\textbf{Predictive modeling results under different feature sets and AI conditions.} 
Binary classification performance \textcolor{red}{(Accuracy/F1/AUC)} for predicting \textit{cognitive load}, \textit{decision confidence and accuracy}. 
We compare three feature settings: \textit{Eye-tracking only}, \textit{User priors only}, and \textit{Multimodal fusion} (eye tracking + user priors). 
For each predicted target, we report overall performance on pooled trials (\textit{All}) and condition-stratified performance on specific \textit{No-AI}, \textit{Correct-AI}, and \textit{Incorrect-AI} trials; \textit{MoE} denotes a condition-aware mixture-of-experts model. 
Boldface indicates the best condition (All/No-AI/Correct-AI/Incorrect-AI/MoE) for each model within a given feature setting.
Red highlights the best-performing values for each predicted target within that given feature setting across conditions.
Model acronyms: LR (Logistic Regression); SVM (Support Vector Machine); RF (Random Forest); ET (ExtraTrees); AdaB (AdaBoost); XGB (XGBoost); MLP (Multi-Layer Perceptron).
}
\label{tab:res_predictions}
\vspace{-4.6mm}
\end{table*}
